On Automating Proofs of Multiplier Adder Trees using the RTL Books

We present an experimental, verified clause processor ctv-cp that fits into the framework used at Arm for formal verification of arithmetic hardware designs. This largely automates the ACL2 proof development effort for integer multiplier modules that exist in designs ranging from floating-point division to matrix multiplication.

==> eptcsdata.tex <==
\providecommand{\firstpage}{51}
\providecommand{\publicationstatus}{Gamboa and Manolios (Eds):\\
ACL2 Workshop 2025\\
EPTCS 423, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.423.5}{10.4204/EPTCS.423.5}}
\pdfoutput=1

